How Hard is Computing Parity with Noisy Communications?

We show a tight lower bound of $\Omega(N \log\log N)$ on the number of transmissions required to compute the parity of $N$ input bits with constant error in a noisy communication network of $N$ randomly placed sensors, each having one input bit and communicating with others using local transmissions with power near the connectivity threshold. This result settles the lower bound question left open by Ying, Srikant and Dullerud (WiOpt 06), who showed how the sum of all the $N$ bits can be computed using $O(N \log\log N)$ transmissions. The same lower bound has been shown to hold for a host of other functions including majority by Dutta and Radhakrishnan (FOCS 2008). Most works on lower bounds for communication networks considered mostly the full broadcast model without using the fact that the communication in real networks is local, determined by the power of the transmitters. In fact, in full broadcast networks computing parity needs $\theta(N)$ transmissions. To obtain our lower bound we employ techniques developed by Goyal, Kindler and Saks (FOCS 05), who showed lower bounds in the full broadcast model by reducing the problem to a model of noisy decision trees. However, in order to capture the limited range of transmissions in real sensor networks, we adapt their definition of noisy decision trees and allow each node of the tree access to only a limited part of the input. Our lower bound is obtained by exploiting special properties of parity computations in such noisy decision trees.

==> protocol_to_xnd.tex <==
\subsection{From bounded protocols to $\xnd$ trees}
\label{sec:protocol_to_xnd}

\begin{lemma}
\label{lem:protocol-to-xnd}
For any $\epsilon$-noise $(n,k,d,D)$-protocol $\Pi$ and any distribution $\mu$ on $(\{0,1\}^n)^k$, 
there is an $(n,k,3D,\epsilon^d)$-$\xnd$ tree $\cT$ such that $\adv_{\oplus,\mu}(\cT)
\geq \adv_{\oplus,\mu}(\Pi)$.
\end{lemma}

\begin{proof}
We will carry out the translation from bounded protocols to $\xnd$ trees via two intermediate models
of communication protocols.

\begin{definition}[Intermediate protocols] \hspace{0.2in}
The following two kinds of protocols are obtained by imposing
restrictions on bounded protocols for decomposed networks of Definition~\ref{def:network-decomposition}.
\begin{description}
\item[Semi-noisy protocol:] An $\epsilon$-noise $(n,k,d,D)$-semi-noisy
protocol differs from an $\epsilon$-noise $(n,k,d,D)$-protocol only in the following
respects.
\begin{enumerate}
\item[(a)] When it is the turn of an input processor to send a message,
it sends only its input bit, whose independent $\epsilon$-noisy copies are
then received by its neighbors.
\item[(b)] A transmission made by an auxiliary processor is not 
subjected to any noise.
\end{enumerate}
\item[Noisy copy protocol:] An $\epsilon$-noise $(n,k,D)$-noisy-copy 
protocol is an $\epsilon$-noise $(n,k,1,D)$-semi-noisy protocol; in other words,
every input processor makes exactly one broadcast of its input bit, so that each 
of its neighbors receives exactly one independent $\epsilon$-noisy copy of this input bit.
\end{description}
\end{definition}

\begin{remark}
In these special kinds of protocols, the messages sent by
the input processors does not depend on the messages these processors
receive.  Thus, we may assume that the input processors make their
transmissions in the beginning of the protocol an appropriate number of
times, and after that the auxiliary processors interact according to
a zero noise protocol.
\end{remark}

\begin{claim}[From  bounded protocol to semi-noisy] 
\label{clm:protocol-to-semi-noisy}
For every function $f:(\{0,1\}^n)^k \rightarrow \{+1,-1\}$,
distribution $\mu$ on $(\{0,1\}^n)^k$ and every $\epsilon$-noise
$(n,k,d,D)$-protocol $\Pi$, there is an $\epsilon$-noise
$(n,k,d,3D)$-semi-noisy protocol $\Pi_1$ such that $\adv_{f,\mu}(\Pi)
\leq \adv_{f,\mu}(\Pi_1)$.
\end{claim}

\begin{claim}[From semi-noisy to noisy-copy]
\label{clm:semi-noisy-to-noisy-copy}
For every function $f:(\{0,1\}^n)^k \rightarrow \{+1,-1\}$,
distribution $\mu$ on $(\{0,1\}^n)^k$ and every $\epsilon$-noise
$(n,k,d,D)$-semi-noisy protocol $\Pi_1$, there is an $\epsilon^d$-noise
$(n,k,D)$-noisy-copy protocol $\Pi_2$ such that
$\adv_{f,\mu}(\Pi_1) \leq \adv_{f,\mu}(\Pi_2)$.
\end{claim}

\begin{claim}[From noisy-copy to $\xnd$ tree]
\label{clm:noisy-copy-to-xnd}
For every function $f:(\{0,1\}^n)^k \rightarrow \{+1,-1\}$,
distribution $\mu$ on $(\{0,1\}^n)^k$ and every $\epsilon$-noise
$(n,k,D)$-noisy-copy protocol $\Pi_2$, there is an
$(n,k,D,\epsilon)$-$\xnd$ tree $\cT$ such that 
$\adv_{f,\mu}(\Pi_2) \leq \adv_{f,\mu}(\cT)$.
\end{claim}

Lemma~\ref{lem:protocol-to-xnd} follows immediately from  
Claims~\ref{clm:protocol-to-semi-noisy},~\ref{clm:semi-noisy-to-noisy-copy} 
and~\ref{clm:noisy-copy-to-xnd}.
\end{proof}

\begin{proof}[Proof of Claim~\ref{clm:protocol-to-semi-noisy}.] 
Fix an $\epsilon$-noise $(n,k,d,D)$-protocol $\Pi$ on a graph $G$. We will construct an
$\epsilon$-noise $(n,k,d,3D)$-semi-noisy protocol $\Pi_1$ on a graph $G_1=(V_1,E_1)$. The graph
$G_1$ will contain $G$ as a subgraph; however, all vertices inherited
from $G$ will correspond to auxiliary processors. In addition, for
each input vertex $v$ of $G$, we will have a new input vertex $v'$ in
$G_1$, which will be connected to $v$ and its neighbors in $G$.
Let $(I = \bigcup_{j=1}^k I_j, A = A_0 \cup \bigcup_{j=1}^k A_j)$ be
the decomposition corresponding to $\Pi$. The decomposition
corresponding to $\Pi_1$ will be $(I' = \bigcup_{j=1}^k I'_j, A' = A_0
\cup \bigcup_{j=1}^k A'_j)$, where $I'_j= \{v': v \in I_j\}$ and $A'_j
= A_j \cup I_j$.  

Suppose $\Pi$ uses $T$ transmissions. For $i=1,2,\ldots,T$ and $v \in V(G)$, let
$b_v[i]$ be the bit received by $v$ when the $i$-th transmission is made;
if $v$ does not receive the $i$-th transmission, we define $b_v[i]$ to be $0$.
The protocol $\Pi_1$ for simulating $\Pi$ will operate in $T$ stages,
one for each transmission made by $\Pi$.  The goal is to ensure that in
the end each auxiliary processor $v$ of $G_1$ constructs a sequence
$b'_v \in \{0,1\}^T$, such that $\langle{b'_v: v \in V(G)} \rangle$ and
$\langle{ b_v : v \in V(G) }\rangle$ (of the protocol $\Pi$) have the
same distribution, for every input in $(\{0,1\}^n)^k$.  This implies
that the outputs of $\Pi'$ and $\Pi$ have the same distribution.
Suppose the first $\ell-1$ stages have been successfully simulated and
$\langle{ b'_v[1,\ldots,\ell-1]: v \in V(G)} \rangle$ have been
appropriately constructed. We now describe how stage $\ell$ is
implemented and $\langle{b'_v[\ell]: v\in V(G) \rangle}$ are
constructed.  If the $\ell$-th transmission in $\Pi$ is made by an
auxiliary processor $v$ in $G$, then it will be simulated in $\Pi_1$
using one noiseless transmission from $v$; if the $\ell$-th transmission is made by an
input vertex $v$ of $G$, then it will be simulated in $\Pi_1$ using two
(noiseless) transmissions from $v$ and one $\epsilon$-noisy transmission
from the corresponding (newly added) input vertex $v'$.

\vspace{0.1in}

{\it $v$ is an auxiliary vertex in $G$}: \hspace{0.2in}
The auxiliary vertex $v$ in $G_1$ operates exactly in
the same fashion as in $G$, and sends a bit $b$, which is received 
without error by all its neighbors. Each neighbor $w \in V(G)$ of $v$
independently sets its bit $b'_w[\ell]$ to be an $\epsilon$-noisy copy of $b$
(using its internal randomness).

\vspace{0.1in}

{\it $v$ is an input vertex in $G$}: \hspace{0.2in} 
The auxiliary vertex $v$ in $G_1$ has all the information that the corresponding input vertex $v$ in $G$
would have had, except the input (which is now given to the new input
vertex $v'$) . So, $v$ transmits (with no noise) two bits, $b_0$ and
$b_1$, corresponding to the two possible input values that $v'$ might
have. Next, the input vertex $v'$ transmits its input $c$; let $c_w$
denote the $\epsilon$-noisy version of $c$ that the neighbor $w \in V(G)$
receives.  Each neighbor $w$ of $v$ now acts as follows: if
$b_0=b_1$, then it sets $b'_w[\ell]$ to be an $\epsilon$-noisy copy of
$b_0$ (using its internal randomness); if $b_0 \neq b_1$, then it 
sets $b'_w[\ell]$ to $b_{c_w}$.
\end{proof}

\begin{proof}[Proof of Claim~\ref{clm:semi-noisy-to-noisy-copy}.]
Let $\Pi_1$ be an $\epsilon$-noise $(n,k,d,D)$-semi-noisy protocol. As remarked
above, all input processors in a semi-noisy protocol can be assumed to
make their transmissions right in the beginning, after which only the
auxiliary processors operate. Thus, each auxiliary processor receives
at most $d$ independent $\epsilon$-noisy copies of the input from each
input processor in its neighborhood. The following lemma of Goyal,
Kindler and Saks~\cite{Goyal05} shows that a processor can generate $d$
independent $\epsilon$-noisy copies of any input from one
$\epsilon^d$-noisy copy. 

\begin{lemma}[Goyal, Kindler and saks~\cite{Goyal05} (Lemma 36)]
Let $t$ be an arbitrary integer, $\epsilon \in (0, 1/2)$ and $\gamma =
\epsilon^t$. There is a randomized algorithm that takes as input a
single bit $b$ and outputs a sequence of $t$ bits and has the property
that if the input is a $\gamma$-noisy copy of $0$ (respectively of
$1$), then the output is a sequence of independent $\epsilon$-noisy
copies of $0$ (respectively of $1$).
\end{lemma}

We  modify the protocol $\Pi_1$ to an $\epsilon^d$-noise $(n,k,D)$-noisy-copy protocol $\Pi_2$ by requiring
that each input processor makes one $\epsilon^d$-noisy transmission of its
input bit. Each auxiliary processor on receiving such a transmission uses its
internal randomness to extract the required $\epsilon$-noisy 
copies. Then onwards the protocol proceeds as before.  
We may now fix internal randomness used by the auxiliary 
processors in such a way that the advantage of the resulting 
protocol for the input distribution $\mu$ 
is at least as good as that of the original protocol. 
Thus, all processors use (deterministic) functions to compute
the bit that they transmit.
\end{proof}

\begin{proof}[Proof of Claim~\ref{clm:noisy-copy-to-xnd}.]
Let $\Pi_2$ be an $\epsilon$-noise $(n,k,D)$-noisy-copy protocol, with the
underlying decomposition $(I = \bigcup_{j=1}^k I_j, A = A_0 \cup
\bigcup_{j=1}^k A_j)$.  We will now show how this protocol can be
simulated using an $(n,k,D,\epsilon)$-$\xnd$ tree $\cT$.  To keep our notation simple, we will
assume (by introducing new edges, if necessary) that (a) all
processors in $A$ are adjacent, and (b) every processor in $A_j$ is
adjacent to every processor in $I_j$. 

Let $T$ be the total number of transmissions in $\Pi_2$.
Let $b_1, b_2, \ldots, b_T$ be the sequence of bits transmitted in $\Pi_2$ by
the auxiliary processors. Suppose, $b_i$ is transmitted by vertex $v \in
I_j$ by computing $g_i(b_1b_2\cdots b_{i-1}, x_j \oplus z_v)$, where
$x_j$ is the the restriction of the input assignment to $I_j$ and
$z_v$ is an $\epsilon$-noisy vector in $\{0,1\}^n$.

The nodes of the $\xnd$ tree $\cT$ are 0-1 sequences of length at most
$T$ (the root is the node at $0$th level and corresponds to the empty sequence). 
The children of the node $b \in \{0,1\}^{i-1}$ $(0 \leq i-1 \leq T-1)$ 
are the two vertices $b0$ and $b1$. Suppose vertex $v \in A_j$ makes the $i$-th
transmission.  The function that $v$ computes to determine what to transmit,
will be used to compute the successor of the nodes at the $i-1$-th
level.  To state this formally, the label of $b \in \{0,1\}^{i-1}$ (at
level $i-1$ in $\cT$) is $(j, h)$, where $h(x_j,z_v) = b \cdot
g_i(b,x_j \oplus z_v)$. (Since our definition requires the function to
return a child of $b$, $h$ returns an extension of $b$ in
$\{0,1\}^i$.)

The set of leaves of $\cT$, $L(\cT)$, is precisely $\{0,1\}^T$. 
Let $a: L(\cT) \rightarrow \{+1,-1\}$ be defined by $a(b_1b_2\cdots b_T) =
(-1)^{b_T}$. Then, it follows from our definitions that
\begin{eqnarray*}
\adv_{\oplus, \mu}(\cT) &\geq& |\E[ \oplus(x) a(\cT(x))]| \\
                        & = &  |\E[ \oplus(x) (-1)^{b_T}]| \\
                        & = &  \adv_{\oplus, \mu} (\Pi_2).
\end{eqnarray*}
\end{proof}

==> tree_rearrangement.tex <==
\subsection{Tree rearrangement}
\label{sec:tree_rearrangement}

Our main observation in this section is that oblivious decision trees
can be assumed to be ordered when the inputs come from a product
distribution, and we wish to approximate the parity function. To show
this we will describe a method for rearranging an arbitrary oblivious
decision tree so that it becomes ordered.

\begin{definition}[Tree rearrangement] \hspace{0.2in}
Let $\cT$ and $\cT'$ be oblivious decision trees for the same set of
inputs.  We say that $\cT'$ is a rearrangement of tree $\cT$ if
\begin{itemize}
\item both trees query each variable the same number of times;
\item the functions labelling vertices of $\cT'$ also appear in
  $\cT$ (up to obvious renaming of children);
 formally, for every vertex $\hv$ in $\cT'$ labelled $(i,
  \hg)$, there is a vertex $v$ in $\cT$ labelled $(i,g)$ in $T$ and a
  bijection $\pi:C_{\hv} \rightarrow C_v$ such that 
  $\forall x \in S_i: \hg(x) = \pi(g(x))$.
\end{itemize}
\end{definition}

\begin{lemma}[Ordering lemma] \hspace{0.2in}
\label{lem:tree-ordering}
Let $\mu$ be a product distribution on some set $S^k$. Let $f: S^k \rightarrow \{+1,-1\}$ 
be of the form $f(x_1,x_2,\ldots,x_k) = h(x_1)h(x_2) \cdots h(x_k)$, where $h: S \rightarrow \{+1,-1\}$. 
Then every oblivious decision tree $\cT$ can be rearranged to obtain an ordered oblivious 
decision tree $\hT$ such that $\adv_{f,\mu}(\hT) \geq \adv_{f,\mu}(\cT).$
\end{lemma}

This lemma will follow immediately from the following claim.

\begin{claim}[Move to root] \hspace{0.2in}
\label{clm:move-to-root}
 Let $\mu$ be a product distribution on $S^k$. Let $f: S^k \rightarrow \{+1,-1\}$ be of the form
$f(x_1,x_2,\ldots,x_k) = h(x_1)h(x_2)\cdots h(x_k)$, where $h: S \rightarrow \{+1,-1\}$. 
Let $\cT$ be an oblivious decision tree with inputs in $S^k$
such that the input $x_n$ is queried only at the level just above the
leaves. Then, $\cT$ can be rearranged to obtain a tree $\hT$ where
\begin{enumerate}
\item the input $x_k$ is queried only at the root;
\item for all $j \neq k$, if $x_j$ was queried at level $r$ of $\cT$,
  then $x_j$ is queried at level $r+1$ of $\hT$;
\item $\adv_{f,\mu}(\hT) \geq \adv_{f,\mu}(\cT)$.
\end{enumerate}
\end{claim}

\begin{proof}
Let $X=\langle{X_1,X_2,\ldots,X_k}\rangle$ take values in $S^k$ with
distribution $\mu$; since $\mu$ is a product distribution the $X_i$'s
are independent. Suppose $\cT$ makes $t$ queries to the input.  Let
$\rv_1, \rv_2, \ldots, \rv_{t+1}$ be the random sequence of vertices
visited by the computation of $\cT$ on input $X$. 
Fix $b: L(\cT) \rightarrow [-1,+1]$ such that 
\begin{eqnarray*}
\adv_{f,\mu}(\cT) & = & |\E[h(X_1)h(X_2)\cdots h(X_k) b(\rv_{t+1})]| \\
                 & = & |\E[\E[h(X_1)\cdots  h(X_k) b(g_{\rv_t}(X_k)) \mid \rv_t]]|.
\end{eqnarray*}

Since $X_k$ is queried only at the end, $h(X_1)\ldots h(X_{k-1})$
and $b(g_{\rv_t}(X_k))$ are independent given $\rv_t$, so 
$\E[h(X_1)\ldots h(X_{k-1}) h(X_k) b(g_{\rv_t}(X_k)) \mid \rv_t]$
$=$ $\E[h(X_1)\ldots h(X_{k-1}) \mid \rv_t] \cdot \E[h(X_k) b(g_{\rv_t}(X_k)) \mid \rv_t]$.

Let $\alpha(v)= \E[h(X_1)\ldots h(X_{k-1}) \mid \rv_t=v]$ and
$\beta(v) = \E[h(X_k) b(g_{\rv_t}(X_k)) \mid \rv_t=v]$.  Let $v^* =
\arg \max \beta(v)$; thus, among the functions labelling vertices that
query $X_k$ (at level $t$), $g_{v^*}$ has the best advantage in the tree
for $h$ under the distribution of $X_k$. It is thus natural to expect
(and not hard to verify) that if we replace all queries to $X_k$ by
this query $g_{v^*}$, the overall advantage can only improve. Once
this is done, the last query does not depend on the previous query,
and can, therefore, be moved to the root. We now present the argument
formally.  We have,
\begin{eqnarray}
\label{eqn:best-query}
\adv_{f,\mu}(\cT) & = & |\E[\alpha(\rv_t) \beta(\rv_t)]| \\
                  & \leq & \E[|\alpha(v_T)|] \cdot |\beta(v^*)|. \nonumber
\end{eqnarray}

We are now ready to describe the rearrangement of $\cT$. Let $\cT^-$
be the subtree of $\cT$ consisting of the first $t$ levels of
vertices; thus vertices where $X_k$ is queried in $\cT$ become leaves
in $\cT^-$.  We first make $|C_{v^*}|$ copies 
of $\cT^-$; we refer to these copies by $\cT^{-}_c$ $(c \in C_{v^*})$, 
and assume that the root of $\cT^{-}_c$ is renamed
$c$. In the new tree $\hT$, we have a root with label $\langle{k,g_{v^*}}\rangle$ 
which is connected to the subtrees $\cT^{-}$.  We
claim that $\adv_{f,\mu}(\hT) \geq \adv_{f,\mu}(\cT)$. Indeed, consider
the function $\hb: L(\hT) \rightarrow [-1,+1]$ that takes the value
$\sign(\alpha(v))b(c)$ on the leaf in $\cT^-_c$ corresponding to
$v \in L(\cT^{-})$. Then, we have
\begin{eqnarray}
\label{eqn:new-tree}
\adv_{f,\mu}(\hT) & \geq & |\E[h(X_1)h(X_2)\cdots h(X_k) \hb(\hv_T)]| \\
                 & = & \E[|\alpha(\rv_T)|] \cdot |\beta(v^*)|. \nonumber
\end{eqnarray}

Claim~\ref{clm:move-to-root} now follows by combining (\ref{eqn:best-query}) and (\ref{eqn:new-tree}).
\end{proof}

We are now ready to show how trees computing the parity function
can be reordered, and prove Lemma~\ref{lem:tree-ordering}. The argument
essentially involves repeated application of Claim~\ref{clm:move-to-root}
to place all queries made to a variable in adjacent
levels. We state the argument formally by considering a carefully
defined {\em minimal counterexample}.

\begin{proof}[Proof of Lemma~\ref{lem:tree-ordering}.]
Fix an oblivious decision tree $\cT$. Let the depth $\cT$ be $r$. We
say that there is an {\em alternation at level $\ell \in \{3,\ldots,r\}$}
of $\cT$ if the variable queried at level $\ell$ is queried at a level
before $\ell-1$ but not at level $\ell-1$. Clearly, a tree with no
alternations is an ordered tree. Among all rearrangements of $\cT$,
let $\hT$ be such that
\begin{enumerate}
\item[(P1)] $\adv_{f,\mu}(\hT) \geq \adv_{f,\mu}(\cT)$;
\item[(P2)] among all $\hT$ satisfying (P1), $\hT$ has the
          fewest alternations;
\item[(P3)] among all $\hT$ satisfying (P1) and (P2), 
          the last alternation in $\hT$ is farthest from the root.
\end{enumerate}
We claim that $\hT$ has no alternations.  Let us assume that $\hT$ has
alternations and arrive at a contradiction.  Let $\hT'$ be the tree
obtained from $\hT$ by merging queries on adjacent levels into one
{\em superquery}. That is, if there are $j$ adjacent levels somewhere
in the tree that query $x_i$, with two outcomes, then we replace these
$j$ levels by a single superquery with $2^j$ outcomes.  Note that the
number of alternations in $\hT'$ is the same as in $\hT$. Let $r'$ be
the number of queries in $\hT'$. We consider two cases:

\vspace{0.1in}

{\it $\cT'$ does not have an alternation at level $r'$}: \hspace{0.2in}
Let $x_1$ be the variables queried at level $r'$.  By Claim~\ref{clm:move-to-root}, we
obtain a tree $\hT''$ where the superquery to $x_1$ appears only at the
root, and all other superqueries are shifted one level down.  Now,
however, if each superquery in $\hT''$ is replaced by its
corresponding subtree of queries from $\hT$, then we obtain a
rearrangement of $\hT$ satisfying (P1) and (P2), but with alternation
at a level farther from the root, contradicting (P3).

\vspace{0.1in}

{\it $\cT'$ has an alternation at level $r'$}: \hspace{0.2in}
Suppose $x_1$ is queried at level $r'$, and the previous query to $x_1$ is at level
$r''< r'$ (with no queries to $x_1$ in the levels $r''+1,
r''+2,\ldots, r'-1$). Now, we apply Claim~\ref{clm:move-to-root} to the
subtrees of $\cT'$ rooted at level $r''+1$, thereby obtaining a
rearrangement $\hT''$, where $x_1$ is now queried at levels $r''+1$
instead of at level $r'$.  Clearly, the resulting tree $\hT''$ has
fewer alternations than $\hT'$. Furthermore, if each superquery in
$\hT''$ is replaced by its corresponding tree of queries from $\hT$,
we obtain a rearrangement of $\hT$. It can be verified that this
rearrangement has advantage at least no worse than $\hT$ but has fewer
alternations---contradicting (P2).
\end{proof}
